Unsupervised Embedding Quality Evaluation

Unsupervised learning has recently significantly gained in popularity, especially with deep learning-based approaches. Despite numerous successes and approaching supervised-level performance on a variety of academic benchmarks, it is still hard to train and evaluate SSL models in practice due to the unsupervised nature of the problem. Even with networks trained in a supervised fashion, it is often unclear whether they will perform well when transferred to another domain. Past works are generally limited to assessing the amount of information contained in embeddings, which is most relevant for self-supervised learning of deep neural networks. This works chooses to follow a different approach: can we quantify how easy it is to linearly separate the data in a stable way? We survey the literature and uncover three methods that could be potentially used for evaluating quality of representations. We also introduce one novel method based on recent advances in understanding the high-dimensional geometric structure of self-supervised learning. We conduct extensive experiments and study the properties of these metrics and ones introduced in the previous work. Our results suggest that while there is no free lunch, there are metrics that can robustly estimate embedding quality in an unsupervised way.

==> figures/data/imagenet-train.tex <==
acc	alpha_req	coherence	n	ne_sum	ne_sum_adj	numerical_rank	pseudo_condition_number	rankme	rankme_adj
86.480000	1.380234	3.398973	768.000000	154.654575	0.201373	66.631755	0.001896	711.846280	0.926883
78.434000	0.751659	3.049712	152.000000	61.914984	0.407335	35.654005	0.021557	148.301800	0.975670
86.794000	1.619046	3.923518	1024.000000	147.001334	0.143556	96.333604	0.010205	919.909259	0.898349
78.934000	0.849477	3.273716	384.000000	112.816793	0.293794	81.180935	0.000015	374.531148	0.975342
65.970000	2.101094	6.030313	256.000000	18.371933	0.071765	1.800892	0.013316	183.310238	0.716056
83.960000	1.322331	3.409165	584.000000	45.520828	0.077947	22.949739	0.000192	533.687806	0.913849
81.568000	1.083729	2.352277	304.000000	50.412159	0.165829	34.982761	0.000346	289.077442	0.950913
75.688000	0.868926	2.707522	192.000000	83.510594	0.434951	74.326681	0.002594	186.928127	0.973584
71.866000	0.943305	2.075710	168.000000	68.690065	0.408869	64.961785	0.003634	162.734869	0.968660
88.586000	1.703504	5.839885	1024.000000	188.426930	0.184011	50.965648	0.005999	910.568968	0.889228
89.204000	1.733721	5.777648	1024.000000	191.016264	0.186539	51.809900	0.005747	908.017521	0.886736
63.100000	1.345049	4.404705	1280.000000	65.216724	0.050951	65.611787	0.100830	1124.717950	0.878686
68.818000	1.305685	4.008852	1280.000000	61.745998	0.048239	60.754363	0.102808	1141.500984	0.891798
72.114000	1.346479	4.944851	1280.000000	51.833995	0.040495	52.365566	0.092005	1138.872590	0.889744
76.530000	1.019238	11.131868	384.000000	2.792532	0.007272	2.798253	0.031492	326.144626	0.849335
77.916000	1.456720	10.997830	1280.000000	45.661377	0.035673	6.909513	0.028971	1067.611300	0.834071
65.246000	1.241427	3.515337	1024.000000	55.609334	0.054306	11.211530	0.026208	928.181181	0.906427
67.652000	1.447437	3.658494	1024.000000	36.426188	0.035572	13.205820	0.045280	875.770756	0.855245
74.644000	1.556537	4.897910	384.000000	14.771448	0.038467	13.632391	0.075244	331.813630	0.864098
68.912000	1.605584	3.578812	320.000000	18.754598	0.058608	18.688597	0.092701	275.085447	0.859642
78.090000	29.600692	3.288292	512.000000	93.677456	0.182964	63.126053	0.000000	249.163229	0.486647
82.594000	23.732065	4.278324	768.000000	163.615705	0.213041	148.979173	0.000000	371.469658	0.483684
84.050000	1.813462	17.906190	1792.000000	28.892023	0.016123	10.152017	0.011616	1500.760803	0.837478
77.858000	1.353293	6.062004	1280.000000	24.563010	0.019190	13.809564	0.041495	1113.074233	0.869589
87.148000	1.675290	10.272430	1536.000000	125.220047	0.081523	12.437661	0.000002	1386.594397	0.902731
78.658000	1.513994	5.459386	1280.000000	23.999249	0.018749	14.600066	0.040489	1111.823047	0.868612
84.048000	1.755118	15.897022	1536.000000	28.460473	0.018529	28.017567	0.040544	1292.879075	0.841718
85.162000	2.247102	26.608781	1792.000000	38.983918	0.021754	38.585503	0.033412	1335.526987	0.745272
86.088000	2.167438	36.051863	2048.000000	34.896251	0.017039	29.121150	0.026937	1504.233967	0.734489
86.452000	2.379381	31.646879	2304.000000	48.996229	0.021266	43.314283	0.026910	1523.182159	0.661103
86.840000	2.563440	34.627920	2560.000000	76.341332	0.029821	28.031921	0.015058	1545.785412	0.603822
78.356000	1.400061	7.234246	1280.000000	29.210188	0.022820	24.768148	0.055449	1112.920605	0.869469
67.922000	1.184020	6.068357	1024.000000	64.351119	0.062843	61.612100	0.115382	940.301081	0.918263
59.856000	1.343309	5.246663	1280.000000	47.899262	0.037421	10.604606	0.038665	1096.332153	0.856509
86.170000	1.509847	3.682371	768.000000	158.475173	0.206348	109.861421	0.036576	695.309937	0.905351
87.218000	1.389165	4.619474	768.000000	187.806108	0.244539	151.721742	0.032975	707.774355	0.921581
83.306000	1.354289	3.632073	768.000000	123.397289	0.160674	101.621449	0.003218	707.108172	0.920714
85.372000	1.303933	3.876411	768.000000	155.008869	0.201834	130.490166	0.001388	714.156808	0.929892
85.250000	1.782643	4.763187	384.000000	43.194124	0.112485	3.777818	0.000016	331.919997	0.864375
86.036000	1.679835	5.527954	512.000000	53.023404	0.103561	3.479699	0.000004	453.753943	0.886238
86.494000	1.553696	5.409594	512.000000	54.957459	0.107339	3.687468	0.000015	456.104007	0.890828
86.790000	2.002072	7.105377	768.000000	36.454887	0.047467	2.669725	0.000000	649.257227	0.845387
77.820000	0.826427	2.215107	128.000000	64.536060	0.504188	45.480561	0.008181	124.813570	0.975106
85.088000	0.934689	4.460495	384.000000	60.653886	0.157953	13.369574	0.000985	366.547684	0.954551
85.556000	0.925035	4.902744	384.000000	49.409247	0.128670	15.595218	0.000756	367.155137	0.956133
82.388000	0.855521	3.174220	192.000000	78.919869	0.411041	22.981015	0.003023	186.105083	0.969297
83.740000	0.857008	3.786395	192.000000	84.825632	0.441800	21.553983	0.003579	185.959069	0.968537


==> figures/data/imagenet-valid.tex <==
acc	alpha_req	coherence	n	ne_sum	ne_sum_adj	numerical_rank	pseudo_condition_number	rankme	rankme_adj	self_clustering
77.582000	2.651201	5.412150	2048.000000	15.514470	0.007575	2.191416	0.003559	1356.064401	0.662141	0.192022
85.236000	1.467827	2.744710	768.000000	103.893235	0.135278	39.236197	0.011302	694.874399	0.904784	0.001747
86.800000	1.474851	2.802403	768.000000	115.090094	0.149857	39.439173	0.011636	695.090652	0.905066	0.001724
87.476000	1.583495	3.387483	1024.000000	123.512891	0.120618	73.434795	0.010366	916.151060	0.894679	0.001199
88.404000	1.620430	3.432773	1024.000000	137.015209	0.133804	63.842359	0.009431	912.076756	0.890700	0.001266
88.598000	1.630799	3.671439	1024.000000	134.628513	0.131473	63.083852	0.009880	910.476624	0.889137	0.001296
86.480000	1.415895	2.578386	768.000000	133.961982	0.174430	61.787915	0.001760	708.855843	0.922989	0.000985
88.386000	1.533614	3.091741	1024.000000	144.295394	0.140913	69.442866	0.002200	930.534818	0.908725	0.000971
79.272000	1.592546	7.048814	2048.000000	38.044625	0.018576	5.278067	0.009261	1756.116004	0.857479	0.034743
86.054000	1.332152	3.464217	768.000000	123.961978	0.161409	20.280500	0.000445	712.901681	0.928257	0.004130
86.484000	1.416495	3.560610	768.000000	85.309222	0.111080	13.408412	0.000001	714.883002	0.930837	0.008251
83.452000	0.914176	2.897682	384.000000	97.885296	0.254910	27.661948	0.001102	370.007871	0.963562	0.002243
85.046000	0.930596	2.946524	384.000000	101.422004	0.264120	24.251019	0.001245	369.333307	0.961805	0.002752
85.460000	0.962231	3.148158	384.000000	117.692490	0.306491	25.567936	0.000383	369.157338	0.961347	0.002371
84.062000	0.932679	3.153993	288.000000	82.457428	0.286311	32.568563	0.000108	278.851530	0.968234	0.001597
78.386000	0.848722	2.336942	192.000000	67.884562	0.353565	40.800235	0.001496	186.899243	0.973434	0.001155
80.966000	0.911983	2.300087	192.000000	72.689798	0.378593	35.740354	0.000482	186.545723	0.971592	0.001375
79.750000	0.830438	2.244931	192.000000	74.464535	0.387836	35.090867	0.004056	186.735724	0.972582	0.001464
82.194000	0.867755	2.511098	192.000000	83.086279	0.432741	31.443739	0.003103	186.360121	0.970626	0.001704
79.088000	1.024203	2.282853	512.000000	60.211182	0.117600	29.423653	0.000115	489.128191	0.955328	0.002253
82.308000	1.036333	3.241182	512.000000	79.745715	0.155753	26.276235	0.000026	490.651015	0.958303	0.002364
77.512000	0.903384	2.215222	320.000000	56.141734	0.175443	24.514512	0.001396	308.155553	0.962986	0.002627
81.268000	0.701149	2.822601	216.000000	49.461813	0.228990	17.821823	0.020589	210.002956	0.972236	0.004222
78.434000	0.774123	2.523512	152.000000	56.172902	0.369559	37.284145	0.022043	148.139455	0.974602	0.001321
82.288000	1.197982	2.909741	768.000000	123.519662	0.160833	27.116966	0.000083	722.608933	0.940897	0.002646
81.426000	1.046805	2.944134	432.000000	73.571057	0.170303	30.557839	0.000498	412.313599	0.954430	0.002081
73.116000	0.894664	2.233377	192.000000	64.286848	0.334827	45.866415	0.002326	186.381261	0.970736	0.001192
76.946000	1.578913	3.108598	1024.000000	4.952324	0.004836	5.035023	0.021294	843.727089	0.823952	0.030861
81.376000	1.604325	5.749256	1536.000000	8.910283	0.005801	3.072861	0.010131	1258.908198	0.819602	0.119337
80.164000	1.611251	4.423725	768.000000	6.873038	0.008949	2.626124	0.015813	609.603936	0.793755	0.146063
77.014000	0.836785	2.625740	320.000000	91.550039	0.286094	83.285923	0.001008	311.234669	0.972608	0.000644
77.216000	0.751963	3.628010	320.000000	89.180220	0.278688	77.517344	0.002276	312.514330	0.976607	0.000550
84.434000	3.316216	4.401094	1024.000000	118.742462	0.115959	31.457116	0.000002	806.497659	0.787595	0.002545
86.280000	1.592400	3.579073	1024.000000	147.093100	0.143646	101.293606	0.008147	921.464294	0.899867	0.000993
86.794000	1.654649	3.694441	1024.000000	133.878268	0.130740	92.875123	0.009540	915.085925	0.893639	0.001032
78.704000	0.857495	3.951147	384.000000	103.532561	0.269616	83.391212	0.000377	372.937202	0.971191	0.000602
78.934000	0.892367	3.297019	384.000000	100.758999	0.262393	81.054686	0.000014	373.376770	0.972335	0.000583
84.846000	6.903382	6.690619	1536.000000	137.096798	0.089256	30.309533	0.000000	884.627421	0.575929	0.002838
87.016000	2.206475	3.225793	1536.000000	142.755519	0.092940	84.479367	0.001043	1303.341617	0.848530	0.001057
87.472000	2.267104	3.484459	1536.000000	151.376680	0.098553	80.167443	0.002145	1289.723465	0.839664	0.001080
81.470000	0.990741	3.194364	640.000000	192.809063	0.301264	89.902409	0.001212	615.119495	0.961124	0.000581
82.858000	1.159473	4.124288	640.000000	149.233167	0.233177	146.377644	0.010924	605.517844	0.946122	0.000694
81.610000	1.011461	3.047605	640.000000	194.996387	0.304682	93.484055	0.000809	614.472661	0.960114	0.000587
80.426000	0.865013	3.257788	512.000000	147.447937	0.287984	89.799839	0.001105	496.257149	0.969252	0.000528
80.464000	0.869784	3.659697	512.000000	145.642123	0.284457	92.532319	0.002413	495.892645	0.968540	0.000529
83.706000	1.796297	3.906324	768.000000	91.572763	0.119235	30.798975	0.000077	686.910462	0.894415	0.002411
85.262000	1.425861	2.593571	768.000000	130.214563	0.169550	55.638042	0.011888	704.890279	0.917826	0.001250
85.778000	1.461553	2.738513	768.000000	119.256305	0.155282	45.539905	0.011775	701.985303	0.914043	0.001435
82.700000	1.293642	3.417808	768.000000	116.160214	0.151250	34.431385	0.000340	713.933559	0.929601	0.001797
78.908000	1.265787	2.213995	768.000000	120.419823	0.156797	58.089239	0.011009	715.031846	0.931031	0.001138
84.080000	1.344381	2.245216	768.000000	95.070261	0.123789	39.384631	0.010177	707.975217	0.921843	0.001609
82.590000	1.113837	4.470698	768.000000	163.049826	0.212304	60.550181	0.000146	730.459135	0.951119	0.000766
87.338000	5.188122	3.569120	2048.000000	139.236806	0.067987	104.948471	0.000103	1363.346391	0.665696	0.001247
87.748000	5.270788	3.990783	2048.000000	141.482569	0.069083	93.656022	0.000169	1339.668355	0.654135	0.001325
81.536000	22.454396	3.785806	576.000000	66.980590	0.116286	46.609073	0.000000	352.146857	0.611366	0.002466
82.332000	22.488445	3.569904	576.000000	67.860181	0.117813	50.271064	0.000000	354.515106	0.615478	0.002239
83.838000	22.525338	3.851491	576.000000	78.468589	0.136230	40.708707	0.000000	354.758485	0.615900	0.002319
82.400000	23.381411	4.168863	672.000000	80.763948	0.120184	42.854054	0.000000	349.286942	0.519772	0.003093
82.518000	22.646701	3.610601	672.000000	58.771074	0.087457	42.029189	0.000000	384.293273	0.571865	0.002849
84.196000	22.651416	3.612447	672.000000	60.152778	0.089513	38.723269	0.000000	387.116835	0.576067	0.002796
73.964000	22.322524	2.340650	384.000000	69.700847	0.181513	45.500638	0.000000	242.272620	0.630918	0.002869
76.980000	22.211093	2.470416	384.000000	57.573520	0.149931	57.554167	0.000000	245.298595	0.638798	0.002456
82.216000	22.867926	3.622630	1152.000000	47.390323	0.041137	36.510593	0.000000	577.710361	0.501485	0.003051
81.020000	22.279613	3.061494	576.000000	79.476874	0.137981	45.215241	0.000000	356.778137	0.619406	0.002366
73.324000	22.215940	6.132180	288.000000	66.150718	0.229690	47.189042	0.000000	183.759846	0.638055	0.003152
80.884000	1.659644	5.946308	1024.000000	16.639376	0.016249	8.302887	0.021971	877.456793	0.856891	0.009219
77.278000	1.605678	4.889771	768.000000	19.808664	0.025793	6.633103	0.024207	660.711927	0.860302	0.016528
80.896000	1.669698	6.438738	1024.000000	16.799978	0.016406	8.397506	0.020233	877.709230	0.857138	0.009041
77.636000	1.608793	4.887816	768.000000	19.743950	0.025708	6.690250	0.025072	660.554398	0.860097	0.016246
82.228000	1.696038	9.315831	1280.000000	13.080141	0.010219	9.473936	0.021279	1091.566928	0.852787	0.006426
82.702000	1.981151	11.799807	1280.000000	15.350586	0.011993	7.827067	0.017091	1045.937176	0.817138	0.020024
83.548000	1.918476	6.409004	1280.000000	14.318682	0.011186	14.902029	0.027465	1053.407895	0.822975	0.006180
81.774000	1.671625	7.241661	1024.000000	15.478755	0.015116	5.725345	0.018274	869.193294	0.848822	0.018413
82.654000	1.807269	7.784900	1280.000000	16.972135	0.013259	9.798658	0.025456	1068.729514	0.834945	0.009448
80.058000	1.351717	6.162733	1024.000000	23.068583	0.022528	11.511549	0.036813	918.527263	0.896999	0.004700
79.574000	1.304098	5.634914	1024.000000	27.582620	0.026936	8.446058	0.026773	924.802550	0.903127	0.009676
80.546000	1.400447	9.178312	2048.000000	28.648851	0.013989	17.036725	0.027152	1805.089312	0.881391	0.002533
80.534000	1.568130	5.671089	1024.000000	16.987553	0.016589	5.035032	0.013191	882.679680	0.861992	0.035691
80.522000	1.548797	6.933507	1024.000000	16.762017	0.016369	5.581850	0.011773	887.795564	0.866988	0.026418
75.578000	3.123824	23.178081	1024.000000	30.066997	0.029362	5.402943	0.000008	774.662163	0.756506	0.035574
77.358000	25.990963	6.553447	2208.000000	46.773028	0.021183	2.317409	0.000000	671.328863	0.304044	0.190200
75.906000	15.572434	6.975910	1664.000000	43.242416	0.025987	2.425545	0.000000	627.811046	0.377290	0.171494
77.286000	15.350644	5.845268	1920.000000	36.494893	0.019008	2.587051	0.000000	686.963037	0.357793	0.149040
76.588000	3.116715	48.109940	1024.000000	30.409622	0.029697	5.742766	0.000000	800.087416	0.781335	0.031227
78.032000	2.612927	7.472389	1024.000000	28.139539	0.027480	2.212290	0.002987	636.845271	0.621919	0.205091
78.510000	2.502051	5.396386	1024.000000	28.769952	0.028096	2.257155	0.006978	671.192883	0.655462	0.196438
79.448000	2.490804	6.908472	1024.000000	30.759687	0.030039	2.088617	0.006304	675.442582	0.659612	0.232533
78.688000	2.625068	9.436142	1024.000000	31.371379	0.030636	2.128878	0.003997	620.763965	0.606215	0.222746
74.630000	2.567001	4.863110	512.000000	23.410490	0.045724	2.054166	0.009307	343.905338	0.671690	0.237086
64.866000	2.100803	4.936137	256.000000	16.279688	0.063593	1.730895	0.012566	179.335415	0.700529	0.333343
65.970000	2.106364	4.330083	256.000000	18.400343	0.071876	1.783840	0.013095	182.670867	0.713558	0.314402
77.032000	2.884026	5.421110	1024.000000	21.222167	0.020725	1.841850	0.004210	579.711926	0.566125	0.294295
78.464000	2.794283	4.947152	1024.000000	12.715967	0.012418	1.830732	0.004918	648.575695	0.633375	0.273664
78.440000	2.708931	3.512650	1024.000000	13.099358	0.012792	1.933501	0.005691	663.096095	0.647555	0.242504
78.246000	2.837434	5.741827	1024.000000	21.399819	0.020898	1.875065	0.004650	590.238690	0.576405	0.282428
67.892000	2.124520	4.201878	256.000000	18.812627	0.073487	1.815570	0.013346	183.826065	0.718071	0.304161
80.156000	18.465418	18.600911	2688.000000	32.391043	0.012050	1.533126	0.000000	633.944986	0.235843	0.432125
79.822000	16.894488	18.532626	2688.000000	32.246296	0.011996	1.518416	0.000000	612.876714	0.228005	0.442243
76.318000	10.749498	6.329715	832.000000	30.048596	0.036116	1.523331	0.000000	317.361541	0.381444	0.436029
79.216000	1.515121	5.240337	832.000000	14.883454	0.017889	1.221296	0.001176	606.619954	0.729111	0.665182
80.008000	16.991509	18.560338	2688.000000	38.279266	0.014241	1.298683	0.000000	465.671698	0.173241	0.597567
79.642000	15.687471	18.170336	2688.000000	30.681974	0.011414	1.527272	0.000000	644.056760	0.239604	0.435650
79.274000	1.698048	4.309127	2048.000000	62.080225	0.030313	24.157863	0.020793	1777.671557	0.868004	0.002709
79.486000	1.616051	4.655984	2048.000000	55.320298	0.027012	30.980327	0.003422	1796.526105	0.877210	0.002378
83.960000	1.356188	2.622016	584.000000	43.718799	0.074861	23.953374	0.000190	531.597384	0.910269	0.004211
81.568000	1.111634	2.286060	304.000000	48.881205	0.160793	35.830032	0.000335	288.353192	0.948530	0.002228
80.456000	0.918336	1.802814	384.000000	105.801103	0.275524	103.829883	0.003800	371.342261	0.967037	0.000653
75.688000	0.891268	2.536405	192.000000	82.652488	0.430482	73.921707	0.002303	186.716224	0.972480	0.001094
71.866000	0.968468	2.377382	168.000000	67.928915	0.404339	64.970065	0.003116	162.517855	0.967368	0.001496
77.698000	1.401934	3.612658	1280.000000	19.373843	0.015136	10.205837	0.031308	1111.386354	0.868271	0.006298
78.794000	1.370659	5.013416	1280.000000	23.440542	0.018313	9.781055	0.023219	1125.639016	0.879405	0.006065
78.236000	1.441589	9.557083	1280.000000	20.741126	0.016204	15.407792	0.045437	1116.823891	0.872519	0.003162
80.612000	1.434261	6.625027	1408.000000	30.248276	0.021483	22.339645	0.052049	1240.904602	0.881324	0.001840
79.916000	1.483094	7.699862	1408.000000	21.519159	0.015283	15.985276	0.043663	1223.357522	0.868862	0.002566
82.242000	1.560631	8.170218	1536.000000	21.462822	0.013973	21.641616	0.025745	1348.383657	0.877854	0.002397
80.858000	1.588348	7.790575	1536.000000	26.925480	0.017530	26.626448	0.047513	1317.443180	0.857710	0.001850
83.428000	1.540019	5.427759	1792.000000	69.419583	0.038739	23.121210	0.030407	1577.451910	0.880275	0.003607
85.888000	1.573313	6.877265	2048.000000	34.873665	0.017028	14.340754	0.025005	1744.684643	0.851897	0.003545
81.316000	1.483249	6.822993	1536.000000	34.367977	0.022375	5.230833	0.013652	1292.731756	0.841622	0.031731
80.300000	1.480686	8.906108	1536.000000	34.401535	0.022397	4.976598	0.013838	1288.204240	0.838675	0.035552
79.252000	1.569295	5.622282	1280.000000	31.066251	0.024271	5.064562	0.011889	1072.078765	0.837562	0.033276
78.066000	1.430143	8.126009	1280.000000	45.470093	0.035524	5.029486	0.015946	1080.304186	0.843988	0.036831
75.000000	1.476963	7.447315	1280.000000	39.856634	0.031138	4.525123	0.015651	1058.611725	0.827040	0.045197
75.484000	1.400827	4.285838	1280.000000	45.005565	0.035161	4.819097	0.019368	1086.094942	0.848512	0.039795
84.808000	2.126180	8.347760	2152.000000	80.365643	0.037345	16.748102	0.020110	1560.951790	0.725349	0.005791
83.808000	1.797259	9.454708	1792.000000	40.606311	0.022660	27.627891	0.025603	1484.303358	0.828294	0.002740
82.348000	1.749351	22.112487	1024.000000	28.283241	0.027620	18.299685	0.041451	857.662169	0.837561	0.004831
79.982000	3.096720	12.984994	1536.000000	8.605178	0.005602	2.073430	0.003185	934.878993	0.608645	0.189623
76.798000	1.198937	5.753307	1024.000000	41.004371	0.040043	4.757772	0.013149	924.091022	0.902433	0.039574
79.320000	1.804971	4.661168	1024.000000	18.442067	0.018010	3.602032	0.007430	841.604331	0.821879	0.061078
89.100000	3.038103	3.901036	1408.000000	64.900411	0.046094	6.191519	0.000013	956.658666	0.679445	0.027333
89.476000	3.048933	4.242303	1408.000000	64.589674	0.045873	5.948827	0.000014	959.894125	0.681743	0.029466
89.568000	2.202163	4.903764	1408.000000	194.956654	0.138464	60.590455	0.002376	1156.722862	0.821536	0.001351
89.796000	2.247660	5.439853	1408.000000	188.561228	0.133921	55.615102	0.002536	1149.819622	0.816633	0.001429
87.938000	2.341429	4.132184	1024.000000	114.368341	0.111688	25.632118	0.000914	848.096995	0.828220	0.002858
88.586000	1.718601	4.189574	1024.000000	176.605546	0.172466	54.882819	0.006249	909.092337	0.887785	0.001282
88.664000	2.424097	4.769618	1024.000000	107.256294	0.104742	22.068224	0.003561	838.620743	0.818966	0.003494
89.204000	1.747117	4.431559	1024.000000	179.645557	0.175435	55.599086	0.006086	906.603891	0.885355	0.001272
75.124000	1.295552	4.879585	1984.000000	40.344392	0.020335	5.493563	0.013750	1702.636108	0.858184	0.029535
79.150000	2.302687	6.094619	1984.000000	83.235116	0.041953	18.307418	0.021525	1534.830645	0.773604	0.004184
79.680000	2.298508	7.911080	1984.000000	93.743436	0.047250	22.014151	0.024125	1545.374848	0.778919	0.003350
82.048000	2.684063	12.598258	1984.000000	100.068694	0.050438	10.100577	0.012130	1456.864368	0.734307	0.012112
84.664000	1.339954	3.595057	768.000000	44.511907	0.057958	19.915447	0.000100	702.245425	0.914382	0.005145
84.394000	1.331350	3.756072	768.000000	42.195694	0.054942	13.186343	0.000005	699.313396	0.910564	0.009532
84.518000	1.375724	3.578852	768.000000	40.884350	0.053235	14.892882	0.000002	698.826016	0.909930	0.008487
85.644000	2.179797	3.839489	1024.000000	52.024902	0.050806	21.466314	0.000000	894.269946	0.873310	0.004400
85.280000	2.053399	3.866613	1024.000000	39.033424	0.038119	15.054938	0.000000	880.866618	0.860221	0.008010
85.538000	2.128827	3.757745	1024.000000	50.500941	0.049317	19.834287	0.000000	893.011036	0.872081	0.004732
82.526000	1.072721	2.734883	384.000000	44.339291	0.115467	13.067150	0.002599	360.311530	0.938311	0.008587
82.172000	1.047388	2.799434	384.000000	38.321337	0.099795	9.312262	0.009813	357.532175	0.931073	0.016640
82.354000	1.062258	2.759016	384.000000	42.168228	0.109813	11.902577	0.010274	358.681174	0.934066	0.010440
82.464000	1.751014	4.854670	1024.000000	27.266070	0.026627	20.604482	0.045763	854.180717	0.834161	0.003976
84.448000	2.424150	6.701271	1024.000000	70.537184	0.068884	29.022188	0.000000	861.247492	0.841062	0.003010
83.884000	1.754860	5.855964	768.000000	86.645154	0.112819	29.260889	0.000001	692.639819	0.901875	0.002501
83.400000	1.377922	6.222142	512.000000	89.094476	0.174013	22.865538	0.000019	481.841847	0.941097	0.003213
81.952000	1.396119	4.925296	512.000000	75.118680	0.146716	20.117928	0.000011	478.969758	0.935488	0.004075
79.714000	1.403047	5.088720	512.000000	53.520904	0.104533	32.748803	0.000096	476.198373	0.930075	0.002346
73.978000	9.605711	39.047216	1280.000000	45.112595	0.035244	4.892589	0.000000	1013.816452	0.792044	0.038659
78.806000	2.219337	5.082558	2048.000000	22.109082	0.010795	2.981630	0.005752	1474.365604	0.719905	0.104754
79.716000	1.794021	13.499185	2048.000000	36.339580	0.017744	3.680838	0.010325	1581.533835	0.772233	0.074999
82.060000	1.875384	3.927058	2048.000000	44.147583	0.021556	5.087904	0.006885	1699.078137	0.829628	0.042100
79.100000	1.858320	4.954569	2048.000000	53.672578	0.026207	3.712932	0.007304	1652.517090	0.806893	0.074847
81.644000	1.560667	9.049486	2048.000000	44.428890	0.021694	26.640976	0.000026	1809.467642	0.883529	0.002557
81.050000	1.998418	7.394663	1536.000000	84.282751	0.054872	5.572785	0.005741	1226.403148	0.798440	0.033260
75.916000	1.469061	4.774016	1280.000000	22.252944	0.017385	17.325609	0.039222	1087.381109	0.849516	0.004658
76.538000	1.477091	3.470988	1280.000000	21.656812	0.016919	19.271335	0.042242	1087.716306	0.849778	0.004641
77.054000	1.477703	5.007820	1280.000000	21.633438	0.016901	19.885686	0.043224	1088.771856	0.850603	0.004641
77.432000	1.562478	6.580347	1280.000000	22.276458	0.017403	22.490390	0.045632	1091.090137	0.852414	0.004355
77.794000	1.569233	6.608262	1280.000000	22.336180	0.017450	22.389757	0.045574	1090.498139	0.851952	0.004474
78.104000	1.642469	6.416883	1280.000000	21.748803	0.016991	15.240829	0.037956	1077.898011	0.842108	0.009198
76.758000	2.719154	6.098843	2048.000000	22.051498	0.010767	1.650773	0.001933	912.589312	0.445600	0.366643
72.342000	2.990824	6.289396	2048.000000	15.748228	0.007690	1.683479	0.001265	902.300160	0.440576	0.352289
75.114000	2.936470	8.486887	2048.000000	16.803826	0.008205	1.740828	0.001621	917.180049	0.447842	0.328060
78.206000	2.716255	7.138510	2048.000000	21.709507	0.010600	1.719414	0.001987	908.478809	0.443593	0.337137
78.450000	2.822969	7.065375	2048.000000	17.969258	0.008774	1.809670	0.001934	922.249153	0.450317	0.298875
78.920000	2.707842	5.525381	2048.000000	20.497011	0.010008	1.756020	0.002151	912.742793	0.445675	0.321447
78.896000	2.744684	6.658646	2048.000000	19.042446	0.009298	1.783573	0.002027	904.798657	0.441796	0.309648
79.300000	2.721677	6.479828	2048.000000	18.706131	0.009134	1.821718	0.002192	910.146672	0.444408	0.296396
79.474000	2.748618	7.018306	2048.000000	18.375787	0.008973	1.854400	0.002186	898.823323	0.438879	0.284170
80.458000	2.787009	7.632694	1536.000000	10.310455	0.006713	2.310497	0.004939	995.120850	0.647865	0.149779
77.440000	2.651224	5.048914	2048.000000	16.108924	0.007866	2.279289	0.004133	1358.169564	0.663169	0.181028
80.168000	2.568008	5.538669	1536.000000	21.457721	0.013970	2.698933	0.003981	1082.750531	0.704916	0.127327
83.552000	1.390375	4.542760	512.000000	92.408318	0.180485	53.440932	0.000052	484.457762	0.946207	0.001049
83.120000	1.194082	4.085315	384.000000	102.411173	0.266696	56.666890	0.000011	368.628511	0.959970	0.000887
81.414000	1.272379	3.465217	384.000000	81.941624	0.213390	63.290218	0.000440	364.552865	0.949356	0.000962
78.970000	1.496958	6.353393	2048.000000	44.796156	0.021873	3.828404	0.011158	1752.829315	0.855874	0.066941
79.096000	1.539442	5.200620	2048.000000	35.366342	0.017269	3.538935	0.009599	1735.696234	0.847508	0.078421
81.166000	1.729811	4.372934	2048.000000	43.662496	0.021320	6.544631	0.012245	1734.747989	0.847045	0.025155
81.544000	1.576090	3.678958	2048.000000	38.375828	0.018738	18.324085	0.021708	1786.108313	0.872123	0.004979
63.100000	1.388615	2.857733	1280.000000	62.920801	0.049157	63.270330	0.078182	1119.251367	0.874415	0.002213
68.818000	1.351126	3.418329	1280.000000	59.954419	0.046839	59.745853	0.092419	1135.998094	0.887499	0.001810
72.114000	1.390212	3.146469	1280.000000	49.721391	0.038845	49.979887	0.060531	1133.655629	0.885668	0.001802
81.310000	1.910753	14.875037	2048.000000	23.425898	0.011438	4.420189	0.000723	1616.680640	0.789395	0.041883
78.382000	1.895048	4.636066	2048.000000	21.476532	0.010487	4.718271	0.008343	1592.041329	0.777364	0.038862
78.660000	1.897127	4.171766	2048.000000	21.146474	0.010325	4.802047	0.009482	1597.310020	0.779937	0.036711
71.744000	2.164755	3.143596	512.000000	15.182062	0.029652	2.090593	0.001627	387.005159	0.755869	0.211411
74.808000	2.433991	4.015987	512.000000	24.587975	0.048023	2.225347	0.007850	367.403494	0.717585	0.198305
77.630000	1.893945	3.394507	2048.000000	20.873827	0.010192	3.688584	0.007616	1549.762954	0.756720	0.066925
80.228000	1.766221	5.462916	2048.000000	14.731931	0.007193	6.206239	0.010902	1694.209076	0.827251	0.015466
77.104000	2.680516	4.523477	2048.000000	9.259755	0.004521	2.054183	0.000520	1170.963248	0.571759	0.200658
79.078000	1.990008	3.896777	2048.000000	31.972040	0.015611	6.338183	0.007221	1627.862634	0.794855	0.022746
76.530000	1.018677	6.141972	384.000000	2.931387	0.007634	2.945940	0.032056	329.094006	0.857016	0.061593
84.860000	5.593976	12.314388	768.000000	135.686687	0.176675	27.753759	0.002190	431.063379	0.561280	0.003462
86.294000	4.399640	11.986178	768.000000	139.195285	0.181244	101.232230	0.022545	410.923199	0.535056	0.002675
87.922000	3.957549	3.658620	768.000000	90.616509	0.117990	84.065320	0.022130	469.146116	0.610867	0.003646
86.598000	4.268480	11.280861	768.000000	132.842267	0.172972	85.004012	0.022307	415.459279	0.540963	0.002862
88.212000	3.918708	3.799420	768.000000	85.552243	0.111396	81.413520	0.022598	470.507760	0.612640	0.003692
84.926000	12.372342	13.748584	1024.000000	121.942595	0.119085	19.839542	0.000006	334.272941	0.326438	0.006084
86.236000	4.146522	14.496729	1024.000000	125.109401	0.122177	67.256392	0.011064	377.310672	0.368467	0.004047
87.992000	4.446057	4.717680	1024.000000	96.471569	0.094211	83.069447	0.013679	545.752987	0.532962	0.003518
86.518000	4.028355	11.905723	1024.000000	116.796403	0.114059	25.483758	0.007627	398.466084	0.389127	0.005335
88.218000	4.467672	4.896719	1024.000000	95.454661	0.093217	91.057329	0.014061	547.125787	0.534303	0.003464
84.434000	3.631997	5.112243	768.000000	118.111361	0.153791	23.582470	0.007126	568.164459	0.739797	0.003584
85.534000	3.926871	9.354695	768.000000	155.245793	0.202143	83.513816	0.026524	523.060923	0.681069	0.001731
86.088000	3.869781	8.623755	768.000000	150.405382	0.195840	102.417853	0.031112	523.774517	0.681998	0.001747
83.398000	1.610324	3.081637	512.000000	73.613391	0.143776	10.641633	0.033154	461.839126	0.902030	0.010332
85.106000	2.914545	5.240667	512.000000	138.752482	0.271001	93.129074	0.048837	413.486599	0.807591	0.001505
85.662000	2.863328	4.849824	512.000000	137.044636	0.267665	83.674213	0.050296	413.525617	0.807667	0.001617
88.306000	5.193995	9.374504	1536.000000	102.294493	0.066598	83.481274	0.006376	624.360378	0.406485	0.003424
88.538000	5.209804	9.759078	1536.000000	108.020159	0.070326	91.165597	0.006579	624.187439	0.406372	0.003398
78.976000	1.483933	6.162789	1536.000000	32.275108	0.021012	4.289402	0.012030	1272.927051	0.828729	0.047350
77.260000	1.449301	5.330402	1536.000000	33.418493	0.021757	4.306460	0.012662	1268.970377	0.826153	0.048076
75.992000	1.406263	5.392116	0.000000	0.000000	0.000000	4.346951	0.012049	1278.125527	0.832113	0.000000
80.476000	1.522606	19.469242	1536.000000	37.170764	0.024200	4.272219	0.012422	1275.459099	0.830377	0.049778
74.658000	1.380362	5.825191	1280.000000	41.491308	0.032415	4.493208	0.016934	1091.916934	0.853060	0.045522
66.206000	1.547105	3.307315	1280.000000	42.174470	0.032949	3.869569	0.013742	1012.153149	0.790745	0.066029
65.942000	1.338095	4.419136	1280.000000	42.001075	0.032813	4.753888	0.018447	1077.202775	0.841565	0.044241
72.970000	1.395431	3.314555	1280.000000	51.232179	0.040025	4.785885	0.016450	1082.685639	0.845848	0.042223
75.036000	1.409117	4.076335	1280.000000	47.656601	0.037232	4.962677	0.016932	1084.835676	0.847528	0.038369
77.284000	1.414385	3.796668	1280.000000	43.010219	0.033602	4.704938	0.018103	1091.458065	0.852702	0.041407
76.516000	1.372545	4.471559	1792.000000	48.274729	0.026939	5.265684	0.016042	1525.049096	0.851032	0.033790
77.916000	1.499648	3.963814	1280.000000	45.397908	0.035467	6.754802	0.021894	1061.490135	0.829289	0.020394
75.766000	1.314482	3.883756	1280.000000	39.389043	0.030773	35.495803	0.049545	1157.658217	0.904420	0.002201
75.634000	1.609601	10.384182	1280.000000	48.147068	0.037615	32.777476	0.061916	1121.245479	0.875973	0.002476
57.890000	1.434034	2.919121	1024.000000	49.503738	0.048343	16.279221	0.041804	896.020752	0.875020	0.006989
65.246000	1.285410	2.877962	1024.000000	53.529846	0.052275	11.445693	0.017648	923.708447	0.902059	0.011754
67.652000	1.484631	2.923161	1024.000000	35.086449	0.034264	12.752204	0.036986	870.941519	0.850529	0.006707
78.312000	1.511778	4.054435	640.000000	22.237284	0.034746	17.735392	0.068250	553.102567	0.864223	0.006321
74.644000	1.579067	3.365856	384.000000	13.992340	0.036438	13.425382	0.073271	330.409539	0.860442	0.009182
68.912000	1.617619	3.155142	320.000000	18.104707	0.056577	17.885380	0.089647	274.395047	0.857485	0.007218
70.140000	26.962349	1.923561	256.000000	60.097874	0.234757	54.133437	0.000000	125.281042	0.489379	0.004897
75.622000	27.115618	2.350494	384.000000	76.101962	0.198182	59.344299	0.000000	187.271041	0.487685	0.003522
78.090000	27.262639	2.349188	512.000000	89.139004	0.174100	65.097743	0.000000	248.684124	0.485711	0.002821
79.684000	27.152759	2.848139	640.000000	86.526851	0.135198	61.025146	0.000000	306.566210	0.479010	0.002548
80.376000	26.246939	2.911690	768.000000	108.591121	0.141395	76.926931	0.000000	355.098502	0.462368	0.002261
82.594000	23.725901	3.088244	768.000000	144.061101	0.187580	117.179468	0.000000	370.450103	0.482357	0.001906
81.478000	23.394884	2.869048	768.000000	148.640914	0.193543	120.475880	0.000000	370.632105	0.482594	0.001908
80.860000	24.972578	3.003482	896.000000	135.174108	0.150864	76.652736	0.000000	394.475565	0.440263	0.002211
82.942000	23.121254	4.212680	896.000000	160.483565	0.179111	142.531656	0.000000	428.081747	0.477770	0.001716
81.944000	22.769430	3.402845	896.000000	170.541468	0.190336	155.233858	0.000000	428.478956	0.478213	0.001717
81.136000	23.687804	3.864320	1024.000000	127.514216	0.124526	68.402252	0.000000	428.737499	0.418689	0.002263
83.394000	23.369122	3.250254	1024.000000	162.686863	0.158874	141.269595	0.000000	484.088842	0.472743	0.001625
82.324000	23.044913	3.227243	1024.000000	176.507231	0.172370	135.102419	0.000000	484.828568	0.473465	0.001635
84.422000	1.393184	5.623306	768.000000	95.660578	0.124558	20.556326	0.000016	716.481213	0.932918	0.004005
85.250000	2.422421	6.610433	1152.000000	114.347507	0.099260	24.049650	0.000002	1009.467237	0.876274	0.003197
83.768000	1.362992	5.146075	768.000000	94.195938	0.122651	25.445404	0.000006	719.414917	0.936738	0.002952
82.404000	1.381666	4.634335	768.000000	74.168116	0.096573	23.852902	0.000008	713.620807	0.929194	0.003411
82.620000	2.843710	11.774479	4032.000000	44.833144	0.011119	4.699514	0.000000	2553.694679	0.633357	0.045371
82.446000	1.186090	3.743714	1024.000000	112.494679	0.109858	20.606300	0.000708	959.573684	0.937084	0.003833
84.144000	1.563470	2.637733	1024.000000	41.391603	0.040421	41.618223	0.000002	927.595502	0.905855	0.002623
81.094000	1.002788	2.861295	576.000000	111.727573	0.193971	34.015384	0.002719	550.939060	0.956491	0.001809
81.996000	1.109614	2.402269	576.000000	34.339038	0.059616	33.828983	0.000026	545.680945	0.947363	0.001795
72.912000	0.953204	2.032872	256.000000	53.550458	0.209181	40.656099	0.001950	246.886649	0.964401	0.001504
74.530000	0.943094	1.899336	256.000000	56.760690	0.221721	53.608216	0.003398	246.710751	0.963714	0.001353
78.182000	0.937474	2.658423	384.000000	92.138458	0.239944	37.623437	0.002668	369.845852	0.963140	0.001499
79.306000	0.979426	2.074847	384.000000	62.079087	0.161664	61.091115	0.013516	368.038304	0.958433	0.001106
82.782000	2.743096	11.215378	4320.000000	60.219825	0.013940	6.675798	0.000000	2740.161260	0.634297	0.023647
82.110000	4.379126	5.248326	768.000000	117.593683	0.153117	39.425276	0.000004	627.628502	0.817225	0.001953
82.462000	4.320365	5.671555	768.000000	118.835720	0.154734	35.945013	0.000014	613.769722	0.799179	0.002225
77.230000	2.169953	3.221475	512.000000	89.041273	0.173909	59.786105	0.000015	467.257733	0.912613	0.001368
80.316000	1.885887	3.444113	512.000000	107.459634	0.209882	42.264398	0.000004	472.864245	0.923563	0.001522
81.416000	1.581301	4.471309	512.000000	85.925187	0.167823	37.471629	0.000335	474.083350	0.925944	0.001861
70.656000	1.054956	2.994569	256.000000	53.337985	0.208352	48.660491	0.005675	244.153039	0.953723	0.001722
78.694000	1.117205	3.657792	512.000000	86.855351	0.169639	39.351225	0.001460	484.993842	0.947254	0.001595
82.076000	1.107469	3.967929	512.000000	110.787482	0.216382	34.522929	0.000106	488.542525	0.954185	0.001629
82.196000	1.152174	5.254179	512.000000	118.931368	0.232288	24.328608	0.000319	484.643676	0.946570	0.003032
83.126000	1.304904	4.635318	512.000000	94.212341	0.184008	23.237212	0.000000	484.276903	0.945853	0.003094
83.716000	1.167128	5.368575	512.000000	99.589341	0.194510	22.587866	0.000006	486.334985	0.949873	0.003191
83.740000	1.160943	5.821045	512.000000	95.269054	0.186072	22.709476	0.000019	486.997617	0.951167	0.003288
84.050000	1.855172	4.892106	1792.000000	23.250093	0.012974	10.904523	0.013154	1488.257054	0.830501	0.011523
79.198000	2.804548	3.707457	2048.000000	11.006394	0.005374	2.246302	0.000745	1106.887116	0.540472	0.164265
78.150000	2.692140	3.924487	2048.000000	8.838678	0.004316	2.178666	0.001176	1092.441504	0.533419	0.165057
77.964000	2.654015	3.661359	2048.000000	10.531388	0.005142	2.159656	0.001706	1106.338325	0.540204	0.178022
78.570000	2.691023	3.443222	2048.000000	8.820606	0.004307	2.215603	0.001765	1131.254644	0.552370	0.158443
79.200000	2.690724	3.690892	2048.000000	10.217061	0.004989	2.251818	0.001029	1146.449778	0.559790	0.159884
77.522000	2.897640	3.671474	2048.000000	11.697417	0.005712	1.973788	0.000815	1039.594143	0.507614	0.225660
78.246000	2.609011	4.358522	2048.000000	8.283768	0.004045	2.200536	0.001708	1142.504807	0.557864	0.154624
82.890000	1.782829	5.579979	2048.000000	20.899012	0.010205	9.795945	0.014852	1713.847197	0.836839	0.006647
75.506000	1.749110	4.143588	2048.000000	15.197408	0.007421	4.417554	0.010510	1565.362268	0.764337	0.042177
83.832000	2.119518	5.458105	2048.000000	30.848644	0.015063	5.560014	0.007110	1565.350264	0.764331	0.028617
84.518000	2.103453	6.438520	2048.000000	39.840407	0.019453	5.281329	0.006936	1580.491651	0.771724	0.033818
78.478000	1.846329	4.398436	2048.000000	20.001382	0.009766	6.820637	0.010605	1609.459377	0.785869	0.017161
80.974000	1.728311	4.600013	2048.000000	20.527366	0.010023	8.439100	0.009924	1694.854842	0.827566	0.008921
80.988000	1.821908	4.271698	2048.000000	23.108046	0.011283	9.123837	0.012285	1674.614725	0.817683	0.009711
81.108000	1.831887	5.389047	2048.000000	25.916102	0.012654	8.384578	0.011281	1675.565366	0.818147	0.011327
77.858000	1.417431	3.822966	1280.000000	22.030053	0.017211	11.889292	0.031568	1100.313771	0.859620	0.004700
81.150000	1.918149	4.529322	1280.000000	43.079087	0.033656	4.050915	0.010893	1060.245865	0.828317	0.063211
80.958000	1.911076	3.840690	1280.000000	70.248131	0.054881	2.804335	0.008074	1044.195431	0.815778	0.131963
77.174000	1.715356	3.839285	1024.000000	12.173839	0.011889	2.876221	0.013769	833.582707	0.814046	0.090158
77.982000	1.701076	4.540227	1280.000000	18.709405	0.014617	4.560303	0.016326	1044.399688	0.815937	0.036171
78.412000	1.758148	3.966717	1024.000000	12.666307	0.012369	3.090826	0.013413	827.042710	0.807659	0.076495
72.974000	1.439249	3.677299	1280.000000	43.227782	0.033772	4.325649	0.017712	1066.480149	0.833188	0.051214
75.448000	1.370665	5.984123	1280.000000	44.331783	0.034634	4.511484	0.014326	1091.617125	0.852826	0.045660
83.406000	1.203250	4.649823	384.000000	75.120881	0.195627	18.331641	0.000072	364.956206	0.950407	0.004155
82.806000	1.135793	5.041461	384.000000	86.282594	0.224694	22.996510	0.000033	367.443485	0.956884	0.002912
82.342000	1.016167	4.543765	384.000000	95.159881	0.247812	27.562690	0.000094	368.876100	0.960615	0.002237
73.038000	1.541460	3.319682	512.000000	19.724617	0.038525	3.228120	0.024620	421.633687	0.823503	0.083019
76.912000	1.456021	3.348146	512.000000	16.239605	0.031718	3.830268	0.028018	437.029260	0.853573	0.050690
80.156000	1.683831	5.903095	2048.000000	16.482699	0.008048	7.297004	0.015695	1735.912152	0.847613	0.008618
74.084000	1.626870	3.691077	0.000000	0.000000	0.000000	3.462788	0.014148	984.647484	0.769256	0.000000
87.148000	1.747565	6.561944	1536.000000	110.914825	0.072210	13.471771	0.000002	1377.132945	0.896571	0.010221
76.848000	1.480527	4.490669	1280.000000	20.713931	0.016183	13.304162	0.036231	1099.253697	0.858792	0.004809
77.086000	1.426923	4.348173	1280.000000	19.839757	0.015500	10.257930	0.036180	1109.847353	0.867068	0.006379
78.658000	1.569641	3.293278	1280.000000	22.813230	0.017823	13.215777	0.036922	1101.743534	0.860737	0.004225
78.826000	1.449879	4.297681	1280.000000	22.006250	0.017192	14.040476	0.038200	1112.239645	0.868937	0.003644
79.280000	1.402246	4.664322	1280.000000	19.243800	0.015034	12.335098	0.043661	1123.924619	0.878066	0.003959
81.388000	1.551957	4.135713	1280.000000	22.788012	0.017803	17.512855	0.041899	1111.116068	0.868059	0.002544
80.086000	1.537212	4.058707	1408.000000	21.112686	0.014995	19.813886	0.047848	1211.488947	0.860432	0.002475
80.300000	1.488727	5.142913	1408.000000	20.474749	0.014542	18.232685	0.048152	1222.447295	0.868215	0.002467
82.380000	1.707018	4.668817	1408.000000	25.389915	0.018033	24.667599	0.043614	1190.525224	0.845543	0.002124
81.636000	1.562274	4.111176	1536.000000	21.119108	0.013749	20.523843	0.044194	1319.670799	0.859161	0.002241
81.822000	1.550349	4.970003	1536.000000	22.970995	0.014955	23.034696	0.047331	1322.582285	0.861056	0.002245
84.048000	1.802608	5.558405	1536.000000	23.712130	0.015438	22.655294	0.035982	1281.368122	0.834224	0.002052
83.022000	1.868945	3.701432	1792.000000	19.263233	0.010750	11.114094	0.023310	1416.989346	0.790731	0.010722
83.248000	1.822699	8.736886	1792.000000	33.986077	0.018965	22.365780	0.037020	1457.231265	0.813187	0.003340
85.162000	2.297082	7.503469	1792.000000	31.681988	0.017680	32.035163	0.029197	1324.232241	0.738969	0.002036
84.252000	1.801983	5.869877	2048.000000	23.748126	0.011596	12.083657	0.024915	1652.080653	0.806680	0.008768
86.088000	2.222211	9.013396	2048.000000	25.872763	0.012633	25.033581	0.024040	1494.930638	0.729947	0.002644
83.812000	1.743448	4.231898	2048.000000	23.738909	0.011591	18.025336	0.031507	1677.523682	0.819103	0.004168
84.110000	2.195318	5.151289	2304.000000	22.326452	0.009690	7.468155	0.011811	1566.841512	0.680053	0.021768
84.788000	2.182468	8.312999	2304.000000	20.375138	0.008843	6.695486	0.012018	1609.665178	0.698639	0.025957
86.452000	2.450221	8.101334	2304.000000	35.366811	0.015350	35.844922	0.023365	1511.507157	0.656036	0.002372
85.120000	2.204991	5.398009	2560.000000	20.826450	0.008135	6.250595	0.010309	1729.853648	0.675724	0.029400
86.840000	2.635524	6.933075	2560.000000	61.887074	0.024175	28.280091	0.014491	1542.338852	0.602476	0.003089
84.936000	2.016673	4.416627	2560.000000	28.917644	0.011296	13.893357	0.018505	1870.206836	0.730550	0.007425
85.370000	2.104064	6.414655	2816.000000	36.903032	0.013105	7.749045	0.011928	1980.847596	0.703426	0.019953
85.370000	2.091809	6.162336	2816.000000	25.028031	0.008888	13.639748	0.016493	1979.207712	0.702844	0.007453
77.306000	1.544660	4.268103	1280.000000	13.829619	0.010804	13.472082	0.037210	1089.873526	0.851464	0.005919
77.908000	1.907962	4.506926	1280.000000	12.158447	0.009499	12.002586	0.028574	1019.336399	0.796357	0.007450
79.308000	1.857476	4.709449	1280.000000	9.459532	0.007390	9.384678	0.023084	1025.973092	0.801541	0.010451
80.250000	1.566755	4.616445	1536.000000	32.310193	0.021035	4.828165	0.009688	1264.361328	0.823152	0.036676
78.130000	1.463519	4.130239	1280.000000	34.006840	0.026568	5.111903	0.011246	1074.193381	0.839214	0.032766
76.594000	1.458270	3.834558	1280.000000	40.919771	0.031969	4.948998	0.008508	1071.734068	0.837292	0.037084
74.830000	1.410431	3.476204	1280.000000	43.943280	0.034331	4.778651	0.019200	1084.960029	0.847625	0.040497
76.642000	1.410360	3.965678	1280.000000	38.218016	0.029858	4.862245	0.017423	1089.777179	0.851388	0.038270
77.468000	1.500986	4.529894	1280.000000	36.199935	0.028281	4.141565	0.017710	1070.223411	0.836112	0.052985
79.820000	1.587625	4.382104	1280.000000	32.288276	0.025225	3.863292	0.011962	1057.057001	0.825826	0.061325
81.536000	1.879294	6.573235	1280.000000	34.139604	0.026672	3.094812	0.007771	985.915895	0.770247	0.102702
78.356000	1.454455	4.411956	1280.000000	26.054280	0.020355	20.899988	0.032815	1102.396649	0.861247	0.002731
79.462000	1.452707	3.858643	1280.000000	25.417145	0.019857	21.634775	0.038331	1104.657319	0.863014	0.002542
80.208000	1.539142	3.655501	1408.000000	23.428916	0.016640	23.417226	0.041659	1188.432845	0.844057	0.002870
81.970000	1.592580	4.744197	1536.000000	24.204147	0.015758	23.798715	0.030123	1281.065683	0.834027	0.002636
82.672000	1.528596	3.387638	1536.000000	49.995705	0.032549	3.028284	0.011097	1259.499398	0.819987	0.113085
85.670000	2.635799	7.394337	1280.000000	56.635526	0.044247	19.481405	0.024391	914.009197	0.714070	0.004339
86.806000	1.641163	6.924565	1280.000000	29.602800	0.023127	7.863146	0.021479	1090.497958	0.851952	0.000000
85.208000	2.518866	6.944257	1280.000000	40.505575	0.031645	16.264365	0.023211	925.236397	0.722841	0.005611
86.004000	1.631821	7.038392	1280.000000	30.086449	0.023505	8.196417	0.022241	1088.049512	0.850039	0.011866
83.894000	2.024438	4.361620	1280.000000	32.044054	0.025034	30.794703	0.043242	946.498288	0.739452	0.002899
84.302000	1.586116	4.300688	1280.000000	31.979785	0.024984	11.045889	0.026090	1083.845863	0.846755	0.006696
86.748000	1.595923	12.021255	1280.000000	51.045957	0.039880	2.491448	0.010656	1064.946278	0.831989	0.166346
77.860000	2.660182	6.281739	2048.000000	16.279435	0.007949	2.284698	0.004102	1357.462636	0.662824	0.180649
78.774000	1.514005	9.031841	1536.000000	35.309439	0.022988	4.922446	0.014441	1283.537039	0.835636	0.036288
76.942000	1.452115	6.550193	1536.000000	39.213349	0.025530	4.801410	0.012077	1282.409361	0.834902	0.038980
75.650000	1.399379	7.532310	1536.000000	38.323270	0.024950	4.537143	0.013198	1284.903154	0.836525	0.044543
73.438000	1.248541	3.786530	1280.000000	48.515949	0.037903	20.911654	0.035399	1161.878000	0.907717	0.004744
75.518000	1.282194	9.363667	1280.000000	40.582870	0.031705	34.682579	0.059404	1158.652930	0.905198	0.001632
72.248000	5.899208	39.062500	1280.000000	43.711374	0.034150	4.795307	0.000000	1073.740960	0.838860	0.040515
65.716000	1.257595	2.737392	1024.000000	66.027855	0.064480	56.445676	0.059397	927.951022	0.906202	0.001639
67.922000	1.227514	3.557357	1024.000000	62.646506	0.061178	58.828584	0.065950	936.176441	0.914235	0.001406
62.906000	8.689062	48.824543	1024.000000	46.034367	0.044955	4.439934	0.000000	817.200754	0.798048	0.050670
77.652000	1.425002	5.512920	1280.000000	17.808501	0.013913	9.953430	0.034170	1108.769500	0.866226	0.006330
74.974000	1.395068	3.714022	1280.000000	22.344133	0.017456	11.038365	0.034407	1103.828042	0.862366	0.006234
71.232000	1.392455	3.213875	1280.000000	30.121349	0.023532	8.784959	0.028848	1089.580295	0.851235	0.010933
66.962000	1.387296	2.997490	1280.000000	36.613848	0.028605	9.198234	0.030009	1090.547836	0.851990	0.010912
59.856000	1.387944	2.830488	1280.000000	47.482816	0.037096	10.177762	0.029030	1090.430369	0.851899	0.010068
81.518000	0.905245	3.063195	384.000000	105.953533	0.275921	31.562716	0.004828	370.311000	0.964352	0.001763
74.738000	12.697925	7.689041	1024.000000	34.498618	0.033690	2.211147	0.000000	417.623105	0.407835	0.204005
82.708000	1.174137	5.642173	512.000000	84.998841	0.166013	35.256184	0.002123	483.078275	0.943512	0.001757
83.140000	1.295399	5.771258	512.000000	87.970103	0.171817	25.286551	0.000943	479.197129	0.935932	0.002905
81.088000	1.140110	5.123481	512.000000	93.409290	0.182440	42.762843	0.000096	485.994312	0.949208	0.001395
83.136000	1.439935	6.046229	768.000000	121.469899	0.158164	26.403173	0.000798	705.866134	0.919097	0.003050
83.678000	2.824995	8.366121	1024.000000	115.892083	0.113176	28.028760	0.000005	826.077708	0.806717	0.003180
81.682000	1.183944	5.937195	512.000000	109.586123	0.214035	33.864315	0.000034	485.654448	0.948544	0.001839
69.024000	1.892366	12.207031	4096.000000	38.065146	0.009293	8.727266	0.000000	3030.078738	0.739765	0.017317
70.360000	3.279859	12.207031	4096.000000	28.227115	0.006891	5.737866	0.000000	2588.699873	0.632007	0.037589
69.926000	1.872749	12.207031	4096.000000	40.934628	0.009994	9.397527	0.000004	3066.290410	0.748606	0.015256
71.594000	3.693145	12.204854	4096.000000	30.689840	0.007493	5.681958	0.000000	2573.337223	0.628256	0.037966
71.594000	1.910856	12.169714	4096.000000	43.778357	0.010688	8.903709	0.000000	3001.055268	0.732680	0.016757
73.350000	4.189637	12.200585	4096.000000	32.477829	0.007929	5.467991	0.000000	2490.177883	0.607954	0.040567
72.368000	1.952895	12.061355	4096.000000	42.873547	0.010467	8.648121	0.000017	2943.846238	0.718712	0.017606
74.214000	5.661464	12.207031	4096.000000	33.627475	0.008210	5.413789	0.000000	2428.403712	0.592872	0.041085
82.106000	1.210857	5.747954	768.000000	91.959978	0.119740	22.182473	0.025323	718.662728	0.935759	0.003223
85.106000	1.716713	5.092767	768.000000	80.670759	0.105040	40.145407	0.009488	679.322904	0.884535	0.001846
79.154000	2.005276	1.696113	768.000000	17.220540	0.022423	17.571966	0.000232	653.649004	0.851105	0.005233
84.532000	1.360883	1.638867	768.000000	19.155948	0.024943	17.476452	0.001366	673.493375	0.876944	0.008443
81.786000	1.699368	3.619638	768.000000	45.484860	0.059225	27.328163	0.000409	682.463845	0.888625	0.003049
80.242000	1.978829	1.856452	768.000000	119.153978	0.155148	3.032159	0.000467	646.433035	0.841710	0.110522
84.268000	1.659362	3.114067	768.000000	130.325816	0.169695	57.846956	0.002264	693.513385	0.903012	0.001288
81.102000	2.022075	1.773594	768.000000	17.422100	0.022685	17.823892	0.000225	652.987513	0.850244	0.005094
86.006000	1.401278	1.682155	768.000000	20.359208	0.026509	18.410985	0.001688	671.503447	0.874353	0.007706
84.210000	1.717768	3.713026	768.000000	47.634804	0.062024	29.111191	0.000439	682.366395	0.888498	0.002794
86.170000	1.528523	3.084401	768.000000	146.657155	0.190960	93.775454	0.033847	693.442583	0.902920	0.001243
85.468000	1.924813	2.574812	768.000000	49.099590	0.063932	11.747407	0.030610	652.261334	0.849299	0.010290
85.930000	1.486988	3.213070	768.000000	147.398410	0.191925	126.063712	0.024949	698.201105	0.909116	0.001133
85.280000	1.846698	2.405392	768.000000	51.145837	0.066596	8.180314	0.006052	656.237097	0.854475	0.018830
87.218000	1.397473	3.822186	768.000000	181.868748	0.236808	146.386521	0.032909	707.340060	0.921016	0.001012
86.620000	1.947771	3.248434	768.000000	74.363367	0.096827	13.939982	0.030329	652.887333	0.850114	0.007475
87.034000	1.480720	3.221580	768.000000	138.778852	0.180702	119.838038	0.021526	697.338009	0.907992	0.001185
86.206000	1.862301	2.789653	768.000000	60.180392	0.078360	7.753773	0.004221	655.368333	0.853344	0.020801
82.202000	1.458522	3.473290	768.000000	128.520845	0.167345	44.510054	0.000292	710.824135	0.925552	0.001265
74.904000	1.716021	1.430904	768.000000	18.454997	0.024030	18.806813	0.000288	677.934648	0.882727	0.004438
80.724000	1.133519	1.678157	768.000000	35.915729	0.046765	21.111862	0.001461	704.558082	0.917393	0.004480
73.690000	1.632431	1.638082	768.000000	106.914585	0.139212	3.205025	0.000073	669.186539	0.871337	0.099027
78.760000	1.729913	2.672587	768.000000	19.195186	0.024994	19.589048	0.000320	677.169642	0.881731	0.004193
83.350000	1.153236	1.587086	768.000000	44.302148	0.057685	20.201295	0.000896	708.485008	0.922507	0.003918
83.306000	1.386059	3.182720	768.000000	115.286700	0.150113	89.138488	0.002891	704.327583	0.917093	0.001137
82.582000	1.836743	4.043750	768.000000	114.424422	0.148990	24.297770	0.018453	673.096459	0.876428	0.003645
81.930000	1.885239	3.410393	768.000000	104.215712	0.135698	28.827095	0.021326	668.675333	0.870671	0.002626
85.372000	1.323134	3.455568	768.000000	141.828808	0.184673	117.018414	0.001250	712.593261	0.927856	0.000953
85.212000	1.362156	2.966536	768.000000	153.463408	0.199822	118.109966	0.003110	710.430721	0.925040	0.000963
85.784000	1.365800	3.365840	768.000000	144.284614	0.187871	121.903967	0.000095	711.231167	0.926082	0.000960
86.212000	1.921990	5.194181	768.000000	68.273422	0.088898	36.587596	0.004652	666.315183	0.867598	0.002116
85.796000	1.370198	1.510407	768.000000	21.379669	0.027838	22.176594	0.001997	674.264264	0.877948	0.006696
84.972000	1.803720	1.567545	768.000000	48.569326	0.063241	38.669996	0.000093	676.101769	0.880341	0.002544
88.246000	1.825511	2.640767	1280.000000	150.434371	0.117527	75.062664	0.013637	1100.645314	0.859879	0.001203
87.594000	2.336683	2.258473	1280.000000	82.882644	0.064752	25.445844	0.031732	989.112943	0.772744	0.003159
88.574000	1.813680	2.548145	1280.000000	162.260736	0.126766	76.693936	0.013245	1104.371112	0.862790	0.001162
87.890000	1.614783	2.471736	1024.000000	187.409459	0.183017	63.547375	0.024756	910.444187	0.889106	0.001235
87.292000	2.179228	2.098310	1024.000000	35.155587	0.034332	9.674588	0.022158	819.824908	0.800610	0.012657
88.168000	1.621396	4.138515	1024.000000	125.697767	0.122752	114.253984	0.008901	904.929969	0.883721	0.001325
87.852000	1.991097	2.500281	1024.000000	28.464287	0.027797	3.822963	0.014793	822.320658	0.803048	0.073330
88.182000	1.583490	2.412950	1024.000000	188.452290	0.184035	73.055067	0.029498	915.691757	0.894230	0.001129
87.848000	2.175246	2.190034	1024.000000	36.250151	0.035401	8.311188	0.020423	819.844098	0.800629	0.016624
88.266000	1.988090	2.686723	1024.000000	31.298243	0.030565	3.803827	0.014803	822.472936	0.803196	0.073930
85.842000	1.749200	1.588434	1024.000000	22.195191	0.021675	22.207729	0.000004	870.906680	0.850495	0.006574
87.080000	1.808351	1.620545	1024.000000	23.254551	0.022710	23.708244	0.000004	865.031719	0.844758	0.006241
81.506000	1.792859	4.493407	1024.000000	54.182609	0.052913	40.229412	0.001904	902.245530	0.881099	0.001919
84.434000	1.360726	1.499889	1024.000000	20.639206	0.020155	20.709951	0.000006	898.831044	0.877765	0.006877
86.184000	1.784905	1.651686	1024.000000	15.493835	0.015131	16.044952	0.000000	823.601069	0.804298	0.011680
84.430000	1.049680	5.065376	512.000000	109.301312	0.213479	95.643069	0.000225	490.901135	0.958791	0.000642
85.536000	1.064144	4.484161	512.000000	121.844629	0.237978	85.779489	0.001542	489.737854	0.956519	0.000693
82.484000	1.437276	3.953490	768.000000	130.554634	0.169993	37.775231	0.000310	709.776023	0.924188	0.001604
82.762000	1.372303	3.620449	768.000000	147.774908	0.192415	42.916423	0.000837	715.191796	0.931239	0.001290
79.480000	1.273411	6.706964	896.000000	148.668521	0.165925	39.043637	0.001378	837.725825	0.934962	0.001700
82.466000	1.036031	3.294833	512.000000	125.975493	0.246046	44.521149	0.000241	490.738509	0.958474	0.001073
82.562000	0.998840	3.680947	512.000000	108.252023	0.211430	36.588637	0.001644	490.906141	0.958801	0.001631
82.298000	1.111180	5.491887	512.000000	90.907368	0.177553	38.225461	0.000447	486.693030	0.950572	0.001525
81.462000	0.976738	3.040899	384.000000	97.271423	0.253311	45.338833	0.002352	369.340069	0.961823	0.001130
78.846000	1.104563	1.293571	384.000000	39.076176	0.101761	17.385757	0.003455	361.453902	0.941286	0.004381
81.402000	1.230921	1.983015	384.000000	30.096527	0.078376	12.810326	0.005025	351.734528	0.915975	0.008294
81.120000	1.113627	1.304660	384.000000	41.343400	0.107665	18.643957	0.003771	361.852930	0.942325	0.003863
83.802000	1.260218	2.103490	384.000000	33.764417	0.087928	12.098105	0.004540	351.065695	0.914234	0.008740
75.990000	1.252883	2.215645	384.000000	26.929498	0.070129	11.445254	0.000873	349.989338	0.911431	0.010159
80.480000	1.286154	2.161041	384.000000	29.467853	0.076739	11.222524	0.000732	349.767551	0.910853	0.010077
81.858000	1.283172	2.554036	384.000000	32.677526	0.085098	17.690239	0.002909	351.157536	0.914473	0.005828
84.046000	1.324894	2.050240	384.000000	24.555368	0.063946	15.192202	0.002668	348.893422	0.908577	0.007379
82.236000	1.130694	4.638606	512.000000	103.553858	0.202254	31.966821	0.000801	485.590543	0.948419	0.001925
81.094000	1.109123	4.124066	384.000000	78.635525	0.204780	35.141716	0.000110	366.334585	0.953996	0.001657
75.454000	1.160697	2.899832	192.000000	25.766096	0.134198	10.552314	0.017652	177.252443	0.923190	0.011533
78.430000	1.179887	2.950548	192.000000	28.751846	0.149749	9.890259	0.014100	177.204742	0.922941	0.012274
71.788000	1.163499	3.188951	192.000000	24.411272	0.127142	10.405318	0.008921	176.899095	0.921349	0.012150
75.952000	1.177317	3.254303	192.000000	27.953598	0.145592	9.935723	0.007135	177.141701	0.922613	0.012388
84.164000	1.738526	3.910147	384.000000	40.043358	0.104280	4.164072	0.000040	334.193558	0.870296	0.053573
85.250000	1.724756	3.979476	384.000000	33.252933	0.086596	3.508477	0.000015	332.306020	0.865380	0.074494
85.196000	1.663484	4.402584	512.000000	47.329441	0.092440	3.579234	0.000007	454.097583	0.886909	0.073486
86.036000	1.635860	4.212889	512.000000	39.427310	0.077006	3.265987	0.000004	453.454853	0.885654	0.087201
85.408000	1.564684	3.328832	512.000000	52.691173	0.102912	3.903280	0.000007	457.549277	0.893651	0.062765
86.494000	1.520769	4.552803	512.000000	42.533318	0.083073	3.491643	0.000016	455.748547	0.890134	0.077182
85.872000	2.001833	4.497533	768.000000	35.013093	0.045590	3.073419	0.000002	649.961036	0.846303	0.100075
86.790000	1.932318	4.111675	768.000000	28.927380	0.037666	2.557405	0.000000	650.377278	0.846845	0.144015
86.068000	1.701966	4.708827	768.000000	34.551556	0.044989	2.597636	0.000001	665.523770	0.866567	0.143169
86.954000	1.637894	4.100758	768.000000	25.955901	0.033797	2.242859	0.000001	660.245829	0.859695	0.190007
87.044000	1.622501	4.411527	768.000000	25.106646	0.032691	2.218026	0.000003	659.476490	0.858693	0.193700
79.052000	1.799631	5.339469	2048.000000	41.977285	0.020497	3.521596	0.008613	1596.758994	0.779667	0.078249
78.516000	2.252731	13.918995	2048.000000	31.639679	0.015449	4.274584	0.007602	1439.189165	0.702729	0.074246
81.958000	2.248730	7.778874	2048.000000	16.084667	0.007854	3.577506	0.004526	1540.178113	0.752040	0.070076
83.180000	2.049842	8.590314	2048.000000	37.052636	0.018092	5.005757	0.006705	1623.269517	0.792612	0.039004
83.130000	2.069379	6.845333	2048.000000	27.366511	0.013363	4.546650	0.005751	1605.731251	0.784048	0.044084
79.874000	2.265339	13.096543	2048.000000	30.339470	0.014814	3.999793	0.007210	1448.724986	0.707385	0.081492
82.896000	2.448180	3.740362	768.000000	97.399203	0.126822	27.163866	0.000020	688.869856	0.896966	0.002565
84.918000	1.840865	3.465378	768.000000	90.996261	0.118485	27.048400	0.000026	696.884879	0.907402	0.002658
85.754000	1.840315	3.745400	768.000000	85.830330	0.111758	23.341318	0.000004	696.214169	0.906529	0.003323
84.392000	2.379355	3.318883	768.000000	119.257485	0.155283	23.016071	0.000025	680.053453	0.885486	0.003777
85.396000	3.318449	3.268210	768.000000	112.428521	0.146391	24.401858	0.000002	669.629813	0.871914	0.003407
86.000000	3.043151	3.426272	768.000000	107.014025	0.139341	22.083999	0.000010	670.000339	0.872396	0.004000
82.636000	1.187371	3.723900	512.000000	112.389223	0.219510	26.075392	0.000009	486.213102	0.949635	0.002504
84.274000	1.163655	4.183288	512.000000	69.298420	0.135348	23.687734	0.000226	484.321990	0.945941	0.003122
85.412000	1.166204	3.827397	512.000000	65.184079	0.127313	21.446983	0.000181	483.675690	0.944679	0.003621
83.734000	1.126091	3.523093	512.000000	87.632063	0.171156	26.200178	0.000035	487.977835	0.953082	0.002558
85.072000	1.131210	3.726751	512.000000	67.051351	0.130960	25.687922	0.000109	484.991425	0.947249	0.002882
85.816000	1.128049	3.870845	512.000000	64.036744	0.125072	24.099962	0.000177	484.487027	0.946264	0.003168
69.954000	0.834557	1.907720	128.000000	54.686419	0.427238	47.597831	0.011534	124.667000	0.973961	0.001115
72.302000	0.823599	1.911187	128.000000	47.832999	0.373695	43.170128	0.008321	124.743933	0.974562	0.001210
75.458000	0.866519	1.958515	128.000000	52.501217	0.410166	43.685495	0.006647	124.563314	0.973151	0.001269
73.914000	0.854188	2.106526	128.000000	57.056727	0.445756	41.684525	0.008832	124.543651	0.972997	0.001257
76.324000	0.831309	2.011080	128.000000	62.163475	0.485652	46.416064	0.008906	124.759180	0.974681	0.001139
77.820000	0.857804	2.153833	128.000000	63.229143	0.493978	45.838118	0.007937	124.621535	0.973606	0.001210
81.974000	0.943090	3.177125	384.000000	73.596059	0.191656	19.134127	0.001588	367.895857	0.958062	0.004339
83.350000	0.985823	3.391168	384.000000	48.335464	0.125874	21.231799	0.001652	366.881619	0.955421	0.003766
84.706000	1.010232	3.602163	384.000000	44.556668	0.116033	18.877313	0.001207	365.867325	0.952779	0.004497
83.344000	0.890480	3.003935	384.000000	59.314075	0.154464	16.157587	0.001111	368.231348	0.958936	0.005937
84.232000	0.919607	3.354998	384.000000	61.166779	0.159288	16.714118	0.001285	367.695952	0.957542	0.005513
85.088000	0.941482	3.397567	384.000000	55.909951	0.145599	15.352061	0.001157	366.637855	0.954786	0.006425
82.580000	0.921076	3.389437	384.000000	69.504657	0.181002	21.642238	0.000678	369.133546	0.961285	0.003286
83.862000	0.929966	3.679119	384.000000	64.513194	0.168003	16.766216	0.001227	367.465338	0.956941	0.005251
85.098000	0.941853	3.556231	384.000000	57.648733	0.150127	15.526658	0.000997	366.707893	0.954968	0.005975
83.838000	0.904656	3.291671	384.000000	75.837828	0.197494	18.902611	0.000711	369.180467	0.961407	0.004284
84.876000	0.908474	3.428338	384.000000	53.033930	0.138109	19.131814	0.001226	368.127928	0.958666	0.004293
85.556000	0.927039	3.752411	384.000000	47.731246	0.124300	17.872092	0.000948	367.292065	0.956490	0.004839
77.120000	0.844248	2.408508	192.000000	50.642189	0.263761	24.943030	0.005006	186.097849	0.969260	0.002376
78.578000	0.860124	2.466664	192.000000	69.381357	0.361361	31.773766	0.004660	186.341495	0.970529	0.001714
80.940000	0.892945	2.624556	192.000000	70.945480	0.369508	29.238006	0.003719	185.973259	0.968611	0.001941
79.694000	0.865219	2.528617	192.000000	66.712335	0.347460	28.605776	0.003786	186.217165	0.969881	0.001927
81.212000	0.840569	2.643149	192.000000	70.513287	0.367257	26.199813	0.003606	186.368685	0.970670	0.002157
82.388000	0.866134	2.915399	192.000000	71.631095	0.373079	24.619053	0.003250	186.054256	0.969033	0.002385
79.444000	0.842041	2.737142	192.000000	61.124744	0.318358	21.489583	0.002609	186.103159	0.969287	0.002982
80.446000	0.882489	2.716170	192.000000	67.335306	0.350705	21.354346	0.004011	185.621759	0.966780	0.003087
82.570000	0.934849	2.897065	192.000000	70.369831	0.366510	19.645942	0.003114	185.004290	0.963564	0.003553
81.900000	0.921432	3.005668	192.000000	64.715296	0.337059	19.343544	0.000496	185.613489	0.966737	0.003495
82.562000	0.821330	2.835187	192.000000	76.856128	0.400292	27.253197	0.004422	186.582234	0.971782	0.001974
83.740000	0.849634	3.253909	192.000000	74.444675	0.387733	23.292317	0.004007	186.103642	0.969290	0.002556


==> figures/imagenet-train.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[group style={
                      group name=myplot,
                      group size= 2 by 4, horizontal sep=0.75cm,vertical sep=1.15cm},height=3.7cm,width=0.55\linewidth,title style={at={(0.5,0.9)},anchor=south},every axis x label/.style={at={(axis description cs:0.5,-0.15)},anchor=north},]
\nextgroupplot[
 	title = {{$\alpha$-ReQ}, $\rho=0.40$},
	ylabel=ACC$\times100$,
	xmode=log,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.4,draw opacity=1] table[x=alpha_req,y=acc] {figures/data/imagenet-train.tex};

\nextgroupplot[
 	title = {{NESum}, $\rho=0.40$},
	%ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.4,draw opacity=1] table[x=ne_sum,y=acc] {figures/data/imagenet-train.tex};

\nextgroupplot[
 	title = {{RankMe}, $\rho=0.21$},
	ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.4,draw opacity=1] table[x=rankme,y=acc] {figures/data/imagenet-train.tex};

\nextgroupplot[
 	title = {{RankMe$^*$}, $\rho=0.00$},
	%ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.4,draw opacity=1] table[x=rankme_adj,y=acc] {figures/data/imagenet-train.tex};

\nextgroupplot[
 	title = {\textbf{\textcolor{cycle2!50!black}{Stable rank}}, $\rho=0.12$},
	ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.4,draw opacity=1] table[x=numerical_rank,y=acc] {figures/data/imagenet-train.tex};

\nextgroupplot[
 	title = {\textbf{\textcolor{cycle2!50!black}{Cond.\ Num.}}, $\rho=-0.48$},
 	xmode=log,
	%ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.4,draw opacity=1] table[x=pseudo_condition_number,y=acc] {figures/data/imagenet-train.tex};

\nextgroupplot[
 	title = {\textbf{\textcolor{cycle2!50!black}{Coherence}}, $\rho=0.30$},
 	xmode=log,
	ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.4,draw opacity=1] table[x=coherence,y=acc] {figures/data/imagenet-train.tex};
\end{groupplot}
\end{tikzpicture}
\vspace{-5mm}
\caption{Representation quality metrics on the ImageNet training set for over 30 pre-trained models. Spearman rank correlation $\rho$ to the test set accuracy displayed per metric in the title. Methods introduced in this work are highlighted in \textbf{\textcolor{cycle2!50!black}{colored bold}}.\label{fig:imagenet-train}}
\end{figure}

==> figures/imagenet-validation.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[group style={
                      group name=myplot,
                      group size= 2 by 4, horizontal sep=0.75cm,vertical sep=1.2cm},height=3.7cm,width=0.55\linewidth,title style={at={(0.5,0.9)},anchor=south},every axis x label/.style={at={(axis description cs:0.5,-0.15)},anchor=north},]
\nextgroupplot[
 	title = {{$\alpha$-ReQ}, $\rho=0.11$},
	ylabel=ACC$\times100$,
	xmode=log,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.1,draw opacity=0.3] table[x=alpha_req,y=acc] {figures/data/imagenet-valid.tex};

\nextgroupplot[
 	title = {{NESum}, $\rho=0.44$},
	%ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.1,draw opacity=0.3] table[x=ne_sum,y=acc] {figures/data/imagenet-valid.tex};

\nextgroupplot[
 	title = {{RankMe}, $\rho=-0.05$},
	ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.1,draw opacity=0.3] table[x=rankme,y=acc] {figures/data/imagenet-valid.tex};

\nextgroupplot[
 	title = {{RankMe$^*$}, $\rho=0.09$},
	%ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.1,draw opacity=0.3] table[x=rankme_adj,y=acc] {figures/data/imagenet-valid.tex};

\nextgroupplot[
 	title = {\textbf{\textcolor{cycle2!50!black}{Stable rank}}, $\rho=0.37$},
	ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.1,draw opacity=0.3] table[x=numerical_rank,y=acc] {figures/data/imagenet-valid.tex};

\nextgroupplot[
 	title = {\textbf{\textcolor{cycle2!50!black}{Cond.\ Num.}}, $\rho=-0.15$},
 	xmode=log,
	%ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.1,draw opacity=0.3] table[x=pseudo_condition_number,y=acc] {figures/data/imagenet-valid.tex};

\nextgroupplot[
 	title = {\textbf{\textcolor{cycle2!50!black}{Coherence}}, $\rho=-0.04$},
 	xmode=log,
	ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.1,draw opacity=0.3] table[x=coherence,y=acc] {figures/data/imagenet-valid.tex};
\nextgroupplot[
 	title = {\textbf{\textcolor{cycle2!50!black}{SelfCluster}}, $\rho=-0.31$},
 	xmode=log,
	%ylabel=ACC$\times100$,
	%xlabel=$d$,
]
\addplot[only marks, color=cycle3,fill opacity=0.1,draw opacity=0.3] table[x=self_clustering,y=acc] {figures/data/imagenet-valid.tex};

\end{groupplot}
\end{tikzpicture}
\vspace*{-5mm}
\caption{Representation quality metrics on the ImageNet validation set of over 1000 pre-trained models. Spearman rank correlation $\rho$ to the test set accuracy displayed per metric in the title. Methods introduced in this work are highlighted in \textbf{\textcolor{cycle2!50!black}{colored bold}}.\label{fig:imagenet-val}}
\vspace*{-3mm}
\end{figure}
